Searches for Gravitational Waves from Known Pulsars at Two Harmonics in the Second and Third LIGO-Virgo Observing Runs

We present a targeted search for continuous gravitational waves (GWs) from 236 pulsars using data from the third observing run of LIGO and Virgo (O3) combined with data from the second observing run (O2). Searches were for emission from the $l=m=2$ mass quadrupole mode with a frequency at only twice the pulsar rotation frequency (single harmonic) and the $l=2, m=1,2$ modes with a frequency of both once and twice the rotation frequency (dual harmonic). No evidence of GWs was found so we present 95\% credible upper limits on the strain amplitudes $h_0$ for the single harmonic search along with limits on the pulsars' mass quadrupole moments $Q_{22}$ and ellipticities $\varepsilon$. Of the pulsars studied, 23 have strain amplitudes that are lower than the limits calculated from their electromagnetically measured spin-down rates. These pulsars include the millisecond pulsars J0437\textminus4715 and J0711\textminus6830 which have spin-down ratios of 0.87 and 0.57 respectively. For nine pulsars, their spin-down limits have been surpassed for the first time. For the Crab and Vela pulsars our limits are factors of $\sim 100$ and $\sim 20$ more constraining than their spin-down limits, respectively. For the dual harmonic searches, new limits are placed on the strain amplitudes $C_{21}$ and $C_{22}$. For 23 pulsars we also present limits on the emission amplitude assuming dipole radiation as predicted by Brans-Dicke theory.

==> macros.tex <==
% a file of results value macros

% macros
%\newcommand{\macro}[1]{\textcolor{red}{#1}\xspace}
\newcommand{\macro}[1]{{#1}\xspace}

% pulsar macros
\newcommand{\NPULSARS}{\macro{236}}
\newcommand{\NHIGHVALUE}{\macro{}}  % number of "high-value" pulsars
\newcommand{\NOTHREEOVERLAP}{\macro{102}}  % number of pulsars with EM observations overlapping only O3

% results macros
\newcommand{\CRABHZEROBAYES}{\macro{\scinum{1.11}{-26}}}     % Crab 95% h0 limit (Bayesian)
\newcommand{\CRABQTTBAYES}{\macro{\scinum{4.61}{32}\,kg\,m$^2$}}  % Crab 95% Q22 limit (Bayesian)
\newcommand{\CRABELLIPTICITYBAYES}{\macro{\scinum{5.96}{-6}}} % Crab 95% ellipticity limit (Bayesian)

% GOT TO HERE THEN STOPPED

\newcommand{\CRABSDBAYES}{\macro{0.013}}                    % Crab spin-down ratio (Bayesian)
\newcommand{\CRABSDFSTAT}{\macro{0.015}}                    % Crab spin-down ratio (F-statistic)
\newcommand{\CRABSDFIVENVEC}{\macro{0.020}}                     % Crab spin-down ratio (5n-vector)
\newcommand{\CRABPOWERBAYES}{\macro{0.017\%}}               % Crab spin-down luminosity ratio (Bayesian)
\newcommand{\CRABPOWERFSTAT}{\macro{0.024\%}}               % Crab spin-down luminosity ratio (F-statistic)
\newcommand{\CRABPOWERFIVENVEC}{\macro{0.042\%}}                  % Crab spin-down luminosity ratio (5n-vector)
\newcommand{\VELAHZEROBAYES}{\macro{\scinum{1.4}{-25}}}     % Vela 95% h0 limit (Bayesian)
\newcommand{\VELAQTTBAYES}{\macro{\scinum{5.9}{33}\,kg\,m$^2$}}  % Vela 95% Q22 limit (Bayesian)
\newcommand{\VELAELLIPTICITYBAYES}{\macro{\scinum{7.6}{-5}}} % Vela 95% ellipticity limit (Bayesian)
\newcommand{\VELAHZEROFSTAT}{\macro{\scinum{2.6}{-25}}}     % Vela 95% h0 limit (F-statistic)
\newcommand{\VELAHZEROFIVENVEC}{\macro{\scinum{2.3}{-25}}}  % Vela 95% h0 limit (5n-vector)
\newcommand{\VELASDBAYES}{\macro{0.042}}                    % Vela spin-down ratio (Bayesian)
\newcommand{\VELASDFSTAT}{\macro{0.078}}                    % Vela spin-down ratio (F-statistic)
\newcommand{\VELASDFIVENVEC}{\macro{0.070}}                 % Vela spin-down ratio (5n-vector)
\newcommand{\VELAPOWERBAYES}{\macro{0.18\%}}                % Vela spin-down luminosity ratio (Bayesian)
\newcommand{\VELAPOWERFSTAT}{\macro{0.61\%}}                % Vela spin-down luminosity ratio (F-statistic)
\newcommand{\VELAPOWERFIVENVEC}{\macro{0.49\%}}             % Vela spin-down luminosity ratio (5n-vector)

\newcommand{\NBELOWSPINDOWN}{\macro{20}}         % pulsars surpassing the spin-down ratio
\newcommand{\NSPINDOWNONETOTEN}{\macro{53}}      % number of pulsars with spin-down ratios between 1 and 10
\newcommand{\NSPINDOWNBELOWTENMSP}{\macro{41}}   % number of MSPs with spin-down ratios below 10

\newcommand{\SMALLESTHZERO}{\macro{\scinum{8.9}{-27}}}      % smallest h0 upper limit
\newcommand{\SMALLESTHZEROPSR}{\macro{J1623\textminus2631}} % pulsar with smallest h0 upper limit
\newcommand{\SMALLESTHZERODIST}{\macro{1.8\,kpc}}           % distance to pulsar with smallest h0 limit
\newcommand{\SMALLESTHZEROFREQ}{\macro{90.3\,Hz}}           % rotation frequency of pulsar with smallest h0 limit

\newcommand{\SMALLESTQTT}{\macro{\scinum{4.5}{29}}}        % smallest Q22 limit
\newcommand{\SMALLESTELLIPTICITY}{\macro{\scinum{5.8}{-9}}} % ellipticity corresponding to smallest Q22 limit
\newcommand{\SMALLESTQTTRATIO}{\macro{3.4}}                % spin-down ratio corresponding to smallest Q22 limit
\newcommand{\SMALLESTQTTPSR}{\macro{J0636+5129}}           % pulsar with smallest Q22 limit
\newcommand{\SMALLESTQTTDIST}{\macro{0.21\,kpc}}           % distance to pulsar with smallest Q22 limit
\newcommand{\SMALLESTQTTFREQ}{\macro{348.6\,Hz}}         % rotation frequency of pulsar with smallest Q22 limit

\newcommand{\SMALLESTCTO}{\macro{\scinum{1.3}{-26}}}          % smallest C21 limit
\newcommand{\SMALLESTCTOPSR}{\macro{J1744\textminus7619}}        % pulsar with smallest C21 limit
\newcommand{\SMALLESTCTOFREQ}{\macro{213.3\,Hz}}         % rotation frequency of pulsar with smallest C21 limit

\newcommand{\SMALLESTMSPSDRAT}{\macro{1.3}}      % smallest spin-down ratio for an MSPs
\newcommand{\SMALLESTMSPSDRATPSR}{\macro{J0711\textminus6830}} % pulsar with smallest spin-down ratio for an MSP
\newcommand{\SMALLESTMSPSDRATDIST}{\macro{0.11\,kpc}} % distance to pulsar with smallest spin-down ratio for an MSP
\newcommand{\SMALLESTMSPSDRATFREQ}{\macro{182.1\,Hz}} % rotation frequency of pulsar with smallest spin-down ratio for an MSP
\newcommand{\SMALLESTMSPSDRATHZERO}{\macro{\scinum{1.5}{-26}}} % h0 limit of pulsar with smallest spin-down ratio for an MSP
\newcommand{\SMALLESTMSPSDRATQTT}{\macro{\scinum{9.3}{29}\,kg\,m$^2$}} % Q22 limit of pulsar with smallest spin-down ratio for an MSP
\newcommand{\SMALLESTMSPSDRATELLIPTICITY}{\macro{\scinum{1.2}{-8}}} % Q22 limit of pulsar with smallest spin-down ratio for an MSP

